Bank Conflict Free Comparison-based Sorting On GPUs

In this paper we present a framework for designing algorithms in shared memory of GPUs without incurring memory bank conflicts. Using our framework we develop the first comparison-based shared memory sorting algorithm that incurs no bank conflicts. It can be used as a subroutine for GPU sorting algorithms to replace current use of sorting networks in shared memory. Using our bank conflict free shared memory sorting subroutine as a black box, we design BCFMergesort, an algorithm for merging sorted streams of data that are larger than shared memory. Our algorithm performs all accesses to global memory in coalesced manner and incurs no bank conflicts during the merge.

==> primitives.tex <==
\section{Primitives}
\label{sec:primitives}
\paragraph{Data transfer between global and shared memory}
Based on Merrill's observations\cite{merrill:scan} we use the following scheme to transfer 
data between global memory and shared memory. The data is cast into
a vector type to increase the GPUs internal load operation size. The requests are split 
in to multiple rounds (the outer {\em for}-loop in Algorithm~\ref{alg:data-transfer}) with 
several vectors being requested to allow the optimizer to reorganize the requests 
to achieve optimal throughput (the two inner {\em for}-loops in Algorithm~\ref{alg:data-transfer}
should be unrolled).
\\
\begin{algorithm}
\caption{Data transfer between global and shared memory}
\label{alg:data-transfer}
\begin{tabbing}
IN\=PU\=T:   Array in \\
OUTPUT: Array out \\
\\
Array temp[TRANSFERS\_PER\_ROUND] \\
\\
FOR round IN 0..ROUNDS\_PER\_PAGE-1 \+ \\
	FOR count IN 0..TRANSFERS\_PER\_ROUND-1 \+ \\
		temp[count] = in[count $\cdot$ blockade's.x + threadIdx.x] \- \\
\\
	FOR count IN 0..TRANSFERS\_PER\_ROUND \+ \\
		out[count $\cdot$ blockDim.x + threadIdx.x] = temp[count]
\end{tabbing}
\end{algorithm}

% \begin{algorithm}
% \caption{Data transfer between global and shared memory}
% \label{alg:data-transfer}
% \begin{algorithmic} 
% \STATE $n_{vec} \leftarrow \mathit{pagesize} / \mathit{width}_{vec}$
% \STATE $\mathit{elements}[\mathit{count}_{ele}]$
% \STATE $\mathit{count} \leftarrow \mathit{threadIdx.x}$
% \WHILE{$\mathit{count} < n_{vec}$}
% \FOR{$i \mathit{\ in\ } 0..\mathit{count}_{ele}-1$}
% \STATE $\mathit{elements}[i] \leftarrow in[count + \mathit{blockDim.x} \cdot i]$
% \ENDFOR
% \FOR{$i \mathit{\ in\ } 0..\mathit{count}_{ele}-1$}
% \STATE $out[count + \mathit{blockDim.x} \cdot i] \leftarrow \mathit{elements}[i]$
% \ENDFOR
% \ENDWHILE
% \end{algorithmic}
% \end{algorithm}

\paragraph{Transposing a matrix in shared memory}
There is no algorithm known to us that transposes an arbitrary matrix in-place with $\OhOf{1}$ 
extra memory. Fortunately, our algorithms operate on either square matrices or $m \times n$-matrices, 
where $m = 2 \cdot n$. That allows us to limit our transposition to square matrices, splitting 
the long matrix into two square matrices and using in-program addressing to concatenate the pieces.
\\
\begin{algorithm}
\caption{Bank-conflict free transposition of a square matrix}
\label{alg:transpose}
\begin{tabbing}
IN\=PU\=T:   Matrix $m$ \\
OUTPUT: Transposed matrix $m^T$ \\
\\
col = threadIdx.x \\
\\
FOR i IN 1..$\text{count}_{\text{cols}}-1$ \+ \\
	row = col + i \\
	IF $\text{row} < \text{count}_{\text{rows}}$ \+ \\
		$\text{element}_1 = $ matrix[col][row] \\
		$\text{element}_2 = $ matrix[row][col] \\
		matrix[col][row] $= \text{element}_2$\\
		matrix[row][col] $= \text{element}_1$
\end{tabbing}
\end{algorithm}
\\
% \begin{algorithm}
% \caption{Bank-conflict free transposition of a square matrix}
% \label{alg:transpose}
% \begin{algorithmic} 
% \STATE $\mathit{element}_1, \mathit{element}_1, \mathit{row}$
% \STATE $\mathit{col} \leftarrow \mathit{threadIdx.x}$
% \FOR{$i \mathit{\ in\ } 1..\mathit{count}_{columns}-1$}
% \STATE $\mathit{row} \leftarrow \mathit{col} + i$
% \IF{$\mathit{row} < \mathit{count}_{rows}$}
% \STATE $\mathit{element}_1 = \mathit{matrix}[\mathit{col}][\mathit{row}]$
% \STATE $\mathit{element}_2 = \mathit{matrix}[\mathit{row}][\mathit{col}]$
% \STATE $\mathit{matrix}[\mathit{row}][\mathit{col}] = \mathit{element}_1$
% \STATE $\mathit{matrix}[\mathit{col}][\mathit{row}] = \mathit{element}_2$
% \ENDIF
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}

This function executes one sweep of the matrix below the main diagonal, using one 
thread per column. Since no two threads are reading $\mathit{element}_1$ from the same 
row at the same time, and the row where $\mathit{element}_2$ comes from is exclusively 
used by one thread, no bank conflicts can occur.

\paragraph{Sorting $w^2$ elements in shared memory without bank conflicts}
ShearSort sorts a matrix of values in snake-like order by first sorting the rows in 
alternating directions and then columns in ascending order. We use the fact that the 
transposition of a square matrix in shared memory simply changes its order from 
column-major to row-major (see Algorithm~\ref{alg:block-sort}). That way our 
implementation can assign one memory bank to each of $w$ threads to sort.
\\
\begin{algorithm}
\caption{Bank-conflict free sorting in shared memory}
\label{alg:block-sort}
\begin{tabbing}
IN\=PU\=T:   $w\times w$-matrix $m$ \\
OUTPUT: Sorted matrix $m$ \\
\\
FOR i IN 1..$\log_2(w)$ \+ \\
	\# Sort the rows of matrix $m$ \\
	sort rows in parallel in snake-like order \\
	transpose($m$) \\
	\# Sort the columns of matrix $m$ \\
	sort rows in parallel \\
	transpose($m$) \- \\
\\
\# Clean up and remove snake-like order \\
sort rows in parallel \\
transpose($m$)
\end{tabbing}
\end{algorithm}
\\
As a further optimization we copy the entire row to the assigned thread's registers
before sorting. That way we can perform the entire run of Batcher's Odd Even Mergesort 
in register space.

% \paragraph{Transforming a $w\times h\cdot w$-matrix}
% To expand our ShearSort implementation to non-square matrices we need a way to 
% transform those matrices from column-major order to row-major order. This is done 
% by first transforming the square $w\times w$ submatrices. The former rows are now
% split into $h$ columns. Now each thread can gather all values that belong to the 
% same row from its assigned memory bank and store them in contiguous space. This 
% works only if $h$ divides $w$ evenly. We use $h$ groups of $w$ threads in this 
% operation.
% \\
% \begin{algorithm}
% \caption{Transformation of a $w\times h\cdot w$-matrix}
% \label{alg:transform}
% \begin{tabbing}
% IN\=PU\=T:   $w\times h\cdot w$-matrix $m$ \\
% OUTPUT: Transformed matrix $m_t$ \\
% \\
% transpose all $h$ square submatrices in parallel \\
% each thread reads its row's columns \\
% transpose all $h$ square submatrices in parallel \\
% \end{tabbing}
% \end{algorithm}

\newpage






















